Synthetic Benchmarks for Scientific Research in Explainable Machine Learning

As machine learning models grow more complex and their applications become more high-stakes, tools for explaining model predictions have become increasingly important. This has spurred a flurry of research in model explainability and has given rise to feature attribution methods such as LIME and SHAP. Despite their widespread use, evaluating and comparing different feature attribution methods remains challenging: evaluations ideally require human studies, and empirical evaluation metrics are often data-intensive or computationally prohibitive on real-world datasets. In this work, we address this issue by releasing XAI-Bench: a suite of synthetic datasets along with a library for benchmarking feature attribution algorithms. Unlike real-world datasets, synthetic datasets allow the efficient computation of conditional expected values that are needed to evaluate ground-truth Shapley values and other metrics. The synthetic datasets we release offer a wide variety of parameters that can be configured to simulate real-world data. We demonstrate the power of our library by benchmarking popular explainability techniques across several evaluation metrics and across a variety of settings. The versatility and efficiency of our library will help researchers bring their explainability methods from development to deployment. Our code is available at https://github.com/abacusai/xai-bench.

==> notes.tex <==

%% todos:



%%%%%%% neurips camera ready
% removed checklist (as told to do) and removed resubmission statement
% added acks section at the end
% openreview: R7vr14ffhF9.pdf R7vr14ffhF9.supplemental.pdf

%%%%%%% arxiv
% same as camera ready

% check we refer to *two* real datasets

%%%% added for the first neurips update
% explainers such as *kernel shap* assume feature independence \cite
% feature attribution values can be in R^D
% we implement both classification and regression.
% discussion in "performance across metrics"
 
%%%%%%%%%%% changes from arxiv back to neurips round2 submission
% add back resubmission statement and its mentions in the intro and conclusion
% add back neurips checklist
% remove preprint option


%%%%%%%%%%%% changes from round2 submission to september arxiv submission:
% remove resubmission statement and its mentions in the intro and conclusion
% remove neurips checklist (it wasn't mentioned anywhere)
% change preprint option to final
% remove the "Preprint. Under review." from style file
% add willie acknowledgments


%%%%%%%%%%%%% old todos

% add infidelity formal definition to the appendix?
% compress the gaussian equation
% find another non-survey citation for monotonicity
% Remove all abbreviations for metrics, or remove texttt for datasets, and add them to metrics
% update the appendix (remove all traces of faith-/+, etc)
% did we include "runtime and hardware details" in section 5 ?


%%%%% notes:

% read sanity checks file:///Users/colinwhite/Downloads/6064-Article%20Text-9289-1-10-20200513.pdf

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% roar:

% the use roar + AUC, normalizing to 0,1
% https://openaccess.thecvf.com/content_CVPRW_2020/papers/w1/Hartley_Explaining_Failure_Investigation_of_Surprise_and_Expectation_in_CNNs_CVPRW_2020_paper.pdf

% SWAG uses roar plots
% https://openaccess.thecvf.com/content/WACV2021/papers/Hartley_SWAG_Superpixels_Weighted_by_Average_Gradients_for_Explanations_of_CNNs_WACV_2021_paper.pdf

% a baseline for shapley ....  uses roar plots
% https://arxiv.org/pdf/2006.04896.pdf
% I think they compute scores but it's unclear how

% mimic uses roar with AUPRC and AUROC
% note that they actually use the bad version of roar
% https://arxiv.org/pdf/2102.06761.pdf

% they maybe use roar, but no details https://arxiv.org/pdf/2001.05371.pdf
% I think they were the ones with a detailed criticism, too

% maybe, unclear https://arxiv.org/pdf/1905.00780.pdf

% original roar's review / rebuttal
% https://papers.nips.cc/paper/2019/file/fe4b8556000d0f0cae99daa5c5c5a410-Reviews.html



%%%%%%%%%%%%%%%%%%%%%%%%%%%%% shapley debate

% Problems with Shapley-value-based explanations as feature importance measures

% Shapley values are arguably the most widely used tool in explainability research
% since the seminal paper that introduced Kernel-SHAP and BF-SHAP, many other works have designed efficient ways of approximating Shapley values.

% benefit: showing that it is the unique method that satisfies certain good properties (axioms


% note that the use of shapley values has recently been debated

% due to the ubiquity of shapley values in explainability research, we felt that our benchmark would not be complete without shapley values. However, we give a disclaimer that there is an ongoing debate in the literature

% furthermore, we recommend that our metric shapley-corr be used only when using a method that attempts to approximate shapley values, such as SHAPR, Kernel-SHAP, etc. If using another type of explainer, one of hte other four metrics is likely more appropriate
%%%% work that just tries to approximate shapley values:

% TreeSHAP ??


% criticism of SHAP is it generates importance weights by marginalizing over a uniform hypercube of values.
% criticism:  \citep{kumar2020problems}

% criticism: they can assign non-zero attributions to features that are not even referenced by the model
% from \citep{sundararajan2020many}
% examples: https://arxiv.org/pdf/1908.08474.pdf
% look further to find specific examples of when shapley is best vs worst.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% observational vs interventional

% shapr says that conditional is better
% they say that observational (unconditional) is better \citep{janzing2020feature}
% that last paper says that they are just different.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% infidelity

% \citep{yeh2019fidelity}

% the optimal explanation for infidelity is a novel combination of two popular explanation methods. By varying the perturbation distribution that defines infidelity, we obtain novel explanations by optimizing infidelity, which we show to out-perform existing explanations in both quantitative and qualitative measurements

% todo: read infidelity
% todo: https://scholar.google.com/scholar?cites=14868848543196386114&as_sdt=2005&sciodt=0,5&hl=en

% uses infidelity
% Evaluating and Aggregating Feature-based Model Explanations
% Evaluating the visualization of what a Deep Neural Network has learned
% MAPLE and LIME, apparently...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% monotonicity

% used by aix360

%  which simply tries to measure if adding more positive evidence increases the probability of classification in the specified class. 
%If the features are (independent) positively correlated with the decision, then the class probabilities should monotonically increase.

% mentions same monotonicity def'n
% Opportunities and Challenges in Explainable Artificial Intelligence (survey)
% Explainable Artificial Intelligence: a Systematic Review (survey)
% A Survey on the Explainability of Supervised Machine Learning (survey)



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% faithfulness
% https://arxiv.org/pdf/1806.07538.pdf
% used by aix360

% Faithfulness intuition: Are “relevant” features truly relevant?

% uses faithfulness
% Sanity Checks for Saliency Metrics (would be a good one to read)
% Model Agnostic Contrastive Explanations for Structured Data (variant)
% Faithful and Customizable Explanations of Black Box Models (variant)

% mentions same faithfulness def'n
% Opportunities and Challenges in Explainable Artificial Intelligence (survey)
% Explainable Artificial Intelligence: a Systematic Review (survey)

% mentions faithful:
% Is Attention Interpretable?
% Explainable Deep Learning: A Field Guide for the Uninitiated
% Explainability in Human-Agent Systems (different type of faithfulness)
% Learning Global Additive Explanations for Neural Nets Using Model Distillation
% The Dangers of Post-hoc Interpretability: Unjustified Counterfactual
% Black Box Explanation by Learning Image Exemplars in the Latent Feature Space
% Visualizing Deep Networks by Optimizing with Integrated Gradients


==> tables/metrics.tex <==
\begin{table}[h]
    \vspace{-2mm}
    \caption{Summary of evaluation metrics. 
    %\textbf{Time} denotes evaluation time complexity excluding that of model retraining. 
    %$n_{val},n_{train}$ denotes number of test and training datapoints. 
    \textbf{Linearity} indicates whether model linearity is an implicit assumption.
    \textbf{Retrain} indicates whether computing a metric requires
    retraining the original model. To compute the evaluation metric on the entire test set,
    the model must be retrained $\Theta(D)$ times.}
    \label{tab:metrics}
    \vspace{2mm}
    \centering
    \begin{tabular}{ccccc}
        \hline
        Metric & Type & Model evaluations & Retrain & Linearity  \\
        \hline
         
        faith+/-  & correlation & $\Theta(D)$ &  & \checkmark \\

        mono+/- & ranking & $\Theta(D)$ &  & \checkmark \\
         
        roar-faith+/- & correlation & $\Theta(D)$ & \checkmark & \checkmark \\
         
        roar-mono+/- & ranking & $\Theta(D)$ & \checkmark & \checkmark \\

        shapley-mse & accuracy & $\Theta(2^D)$ &  & \\
         
        shapley-corr & correlation & $\Theta(2^D)$ &  & \\
        \hline
    \end{tabular}
\end{table}
